Input optics systems of the KAGRA detector during O3GK

KAGRA, the underground and cryogenic gravitational-wave detector, was operated for its solo observation from February 25th to March 10th, 2020, and its first joint observation with the GEO 600 detector from April 7th -- 21st, 2020 (O3GK). This study presents an overview of the input optics systems of the KAGRA detector, which consist of various optical systems, such as a laser source, its intensity and frequency stabilization systems, modulators, a Faraday isolator, mode-matching telescopes, and a high-power beam dump. These optics were successfully delivered to the KAGRA interferometer and operated stably during the observations. The laser frequency noise was observed to limit the detector sensitivity above a few kHz, whereas the laser intensity did not significantly limit the detector sensitivity.

==> ORCID.tex <==
\section{ORCID}
The list of ORCIDs in the KAGRA Database (as of 2020 August 30)\\~\\

\noindent
Tomotada Akutsu	ORCID: https://orcid.org/0000-0003-0733-7530\\
Akito Araya	ORCID: https://orcid.org/0000-0002-6884-2875\\
Sangwook Bae	ORCID: https://orcid.org/0000-0003-2429-3357\\
Yutaro Enomoto	ORCID: https://orcid.org/0000-0001-6426-7079\\
Nobuyuki Kanda	ORCID: https://orcid.org/0000-0001-6291-0227\\
Chunglee Kim	ORCID: https://orcid.org/0000-0003-3040-8456\\
Keiko Kokeyama ORCID: https://orcid.org/0000-0002-2896-1992\\
Albert Kong	ORCID: https://orcid.org/0000-0002-5105-344X\\
Hyung Won Lee	ORCID: https://orcid.org/0000-0002-1998-3209\\
Ray-Kuang Lee	ORCID: https://orcid.org/0000-0002-7171-7274\\
Chun-Che (Lupin) Lin	ORCID: https://orcid.org/0000-0003-4083-9567\\
Chun-Yu Lin	ORCID: https://orcid.org/0000-0002-7489-7418\\
Yuta Michimura	ORCID: https://orcid.org/0000-0002-2218-4002\\
Kouji Nakamura	ORCID: https://orcid.org/0000-0001-6148-4289\\
Hiroyuki Nakano	ORCID: https://orcid.org/0000-0001-7665-0796\\
Lan Nguyen Quynh	ORCID: https://orcid.org/0000-0002-1828-3702\\
Wei-Tou Ni	ORCID: https://orcid.org/0000-0001-6792-4708\\
John J.~Oh	ORCID: https://orcid.org/0000-0001-5417-862X\\
June Gyu Park	ORCID: https://orcid.org/0000-0002-7510-0079\\
Hisaaki Shinkai	ORCID: https://orcid.org/0000-0003-1082-2844\\
Ayaka Shoda	ORCID: https://orcid.org/0000-0002-0236-4735\\
Edwin J.~Son	ORCID: https://orcid.org/0000-0002-9234-362X\\
Satoshi Tanioka	ORCID: https://orcid.org/0000-0003-3321-1018\\
Flavio Travasso	ORCID: https://orcid.org/0000-0002-4653-6156\\
Tomoyuki Uehara	ORCID: https://orcid.org/0000-0003-4375-098X\\
Helios Vocca	ORCID: https://orcid.org/0000-0002-1200-3917\\
Kohei Yamamoto	ORCID: https://orcid.org/0000-0002-5064-4619\\
Takahiro Yamamoto	ORCID: https://orcid.org/0000-0002-0808-4822\\
Zong-Hong Zhu	ORCID: https://orcid.org/0000-0002-3567-6743



